Harmonic Decomposition in Data Sketches

In the turnstile streaming model, a dynamic vector $\mathbf{x}=(\mathbf{x}_1,\ldots,\mathbf{x}_n)\in \mathbb{Z}^n$ is updated by a stream of entry-wise increments/decrements. Let $f\colon\mathbb{Z}\to \mathbb{R}_+$ be a symmetric function with $f(0)=0$. The \emph{$f$-moment} of $\mathbf{x}$ is defined to be $f(\mathbf{x}) := \sum_{v\in[n]}f(\mathbf{x}_v)$. We revisit the problem of constructing a \emph{universal sketch} that can estimate many different $f$-moments. Previous constructions of universal sketches rely on the technique of sampling with respect to the $L_0$-mass (uniform samples) or $L_2$-mass ($L_2$-heavy-hitters), whose universality comes from being able to evaluate the function $f$ over the samples. In this work we take a new approach to constructing a universal sketch that does not use \emph{any} explicit samples but relies on the \emph{harmonic structure} of the target function $f$. The new sketch ($\textsf{SymmetricPoissonTower}$) \emph{embraces} hash collisions instead of avoiding them, which saves multiple $\log n$ factors in space, e.g., when estimating all $L_p$-moments ($f(z) = |z|^p,p\in[0,2]$). For many nearly periodic functions, the new sketch is \emph{exponentially} more efficient than sampling-based methods. We conjecture that the $\textsf{SymmetricPoissonTower}$ sketch is \emph{the} universal sketch that can estimate every tractable function $f$.

==> pool.tex <==


\subsection{}
We introduce a simple sketch called the \SymmetricPoissonTower.
It is parameterized by an integer $m=\epsilon^{-2}$ 
and maintains a 
vector $(X_k)_{k\in [a,b)}$ of integers, 
where $a=-\Theta(m\log n),b=\Theta(m\log n)$.
In the pseudocode below, 
$Y_{k,v}$, $v\in [n], k\in \Z$, 
is distributed as $Y_{k,v}\sim \SymmetricPoisson(e^{-k/m})$.\footnote{$\SymmetricPoisson(\lambda)$ is the distribution of the difference of two independent $\Poisson(\lambda/2)$ variables.}
The $\Update(v,\Delta)$ function is implemented as follows

\medskip
\centerline{\framebox{
\begin{minipage}{5in}
\begin{tabbing}555\=555\=555\=555\=\kill
$\Update(v,\Delta)$ : $v\in [n], \Delta\in \Z$\\
\>For each $k\in [a,b)$, \ $X_k \gets X_k + \Delta\cdot Y_{k,v}$
\end{tabbing}
\end{minipage}
}}
\medskip 

We prove that the \SymmetricPoissonTower{} is 
$\mathcal{F}$-universal for the function class
\[
\mathcal{F}= \left\{f(x)=cx^2+\int_0^\infty (1-\cos (xs))\,\nu(ds) \;\;\middle|\;\; \begin{array}{l}
\mbox{$c\geq 0, \nu$ is a positive measure, and}\\
\mbox{$\int_0^\infty \min(s^2,1)\,\nu(ds) \leq \poly(nM\epsilon^{-1})\xi(f,M)$,}\\
\mbox{where $\xi(f,M)= \min_{x\in [M]}\{f(x)\mid f(x)>0 \} $}
\end{array}\right\}.
\]
which includes $L_p$ moments, $p\in [0,2]$, 
$\ln(1+|x|)$,
many nearly periodic functions like $g_{np}$,
and the symmetric version of the ``soft cap'' functions studied by Cohen~\cite{cohen2017hyperloglog}.
The total space complexity is 
$O(m\log^2(nMm))=O(\epsilon^{-2}\log^2(nM\epsilon^{-1}))$ bits.

 (The random variables $(Y_{k,v})$ are mutually independent, generated by the random oracle $H$.)
The tractability results in \cite{bar2004information,braverman2010zero,braverman2016streaming} 
apply to the random oracle model, as do all lower bound 
reductions to problems in communication complexity, 
which assume public randomness.

\paragraph{Organization of \S 1.}
In \cref{sec:harmonic} we introduce harmonic moments,
explain why previous approaches cannot 
approximate most of the harmonic moments, and analyze a simple 
1-cell version of the \SymmetricPoissonTower.
In \cref{sec:combine} we illustrate how harmonic moments
can be combined to yield many natural, well studied functions,
and how estimators for harmonic moments can be combined 
with good estimation guarantees.
\cref{sec:choose_t} gives an informal development
of the harmonic moment estimators,
and in \cref{sec:new-results} 
we give a formal presentation of
the \SymmetricPoissonTower's guarantees and other new results.

\subsection{}
 By computation around ($\star\star$), we know if a function can be written as
\begin{align*}
    f(z) &= \int_0^{2\pi} (e^{i\gamma z}-1) \,\mu(d\gamma),
\end{align*}
for some signed measure $\mu$, then the $f$-moment can be estimated by first estimating the $e^{i\gamma z}$-moments for $\gamma \in[0,2\pi)$ and then combining them with the following identity. 
\begin{align*}    \underbrace{\sum_{v\in[n]}f(\mathbf{x}_v)}_{\text{$f$-moment}} &= \int_0^{2\pi} \underbrace{\sum_{v\in[n]}(e^{i\gamma \mathbf{x}_v}-1)}_{\text{$e^{i\gamma z}$-moment}} \,\mu(d\gamma).
\end{align*}

\subsection{}
Braverman and Ostrovsky \cite{braverman2010zero} succeeding in characterizing the class of tractable, increasing functions $f$, using the $L_2$-heavy hitter based sketch.\footnote{Since $f$ is assumed to be symmetric and $f(0)=0$, we say a function $f$ is \emph{increasing} if it increases on $\N$; it is \emph{decreasing} 
if it decreases on $\Z_+$.}
Roughly speaking, $f$ must grow no faster than quadratic, even locally. Braverman and Chestnut~\cite{braverman2015universal} 
characterized all tractable decreasing functions using the uniform sampling based sketch. 
Finally, Braverman, Chestnut, Woodruff, and Yang \cite{braverman2016streaming} characterized generic, 
tractable $f$ outside of the 
class of ``nearly periodic'' functions by combining the techniques in \cite{braverman2010zero,braverman2015universal}.
As a natural byproduct of the strategy, the sketches in \cite{braverman2010zero,braverman2015universal,braverman2016streaming} are all \emph{universal} \cite{braverman2010zero} for their respective function 
classes. We now discuss in greater detail the previous techniques for building universal sketches over turnstile streams.
